Evolution of Retrograde Orbiters in an AGN Disk

AGN disks have been proposed as promising locations for the mergers of stellar mass black hole binaries (BBHs). Much recent work has been done on this merger channel, but the majority focuses on stellar mass black holes (BHs) orbiting in the prograde direction. Little work has been done to examine the impact of retrograde orbiters (ROs) on the formation and mergers of BBHs in AGN disks. Quantifying the retrograde contribution is important, since roughly half of all orbiters should initially be on retrograde orbits when the disk forms. We perform an analytic calculation of the evolution of ROs in an AGN disk. Because this evolution could cause the orbits of ROs to cross those of prograde BBHs, we derive the collision rate between a given RO and a given BBH orbiting in the prograde direction. In the examples given here, ROs in the inner region of the disk experience a rapid decrease in the semimajor axis of their orbits while also becoming highly eccentric in less than a million years. This rapid orbital evolution could lead to extreme mass ratio inspirals detectable by the Laser Interferometer Space Antenna. The collision rates of our example ROs with prograde BBHs in the migration trap depend strongly on the volume of the inner radiation-pressure-dominated region which depends on the mass of the supermassive black hole (SMBH). Rates are lowest for larger mass SMBHs, which dominate the AGN merger channel, suggesting that merger rates for this channel may not be significantly altered by ROs.

==> bh_bib.ltx <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Amy Secunda at 2020-03-11 15:12:40 -0400 


%% Saved with string encoding Unicode (UTF-8) 



@article{FAbj_2020,
	Author = {Fabj, G. and Nasim, S.S. and Caban, F. and {Ford}, K.~E.~S. and {McKernan}, B. and {Bellovary}, J.},
	Date-Added = {2020-03-11 15:11:05 -0400},
	Date-Modified = {2020-03-11 15:12:40 -0400},
	Journal = {in prep.},
	Title = {Aligning stellar and stellar remnant orbits with the plane of an AGN disk},
	Year = {2020}}

@article{Bartos_2017,
	Author = {Bartos, I. and Haiman, Z. and Marka, Z. and Metzger, B. D. and Stone, N. C. and Marka, S.},
	Date-Added = {2020-03-09 13:40:55 -0400},
	Date-Modified = {2020-03-09 13:40:55 -0400},
	Doi = {10.1038/s41467-017-00851-7},
	Issn = {2041-1723},
	Journal = {Nature Communications},
	Month = {Oct},
	Number = {1},
	Publisher = {Springer Science and Business Media LLC},
	Title = {Gravitational-wave localization alone can probe origin of stellar-mass black hole mergers},
	Url = {http://dx.doi.org/10.1038/s41467-017-00851-7},
	Volume = {8},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/s41467-017-00851-7}}

@article{Takahashi_2003,
	Author = {Takahashi, Ryuichi and Nakamura, Takashi},
	Date-Added = {2020-02-26 14:07:58 -0500},
	Date-Modified = {2020-02-26 14:07:58 -0500},
	Doi = {10.1086/377430},
	Issn = {1538-4357},
	Journal = {The Astrophysical Journal},
	Month = {Oct},
	Number = {2},
	Pages = {1039--1051},
	Publisher = {IOP Publishing},
	Title = {Wave Effects in the Gravitational Lensing of Gravitational Waves from Chirping Binaries},
	Url = {http://dx.doi.org/10.1086/377430},
	Volume = {595},
	Year = {2003},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/377430}}

@article{Nakamura_1998,
	Author = {Takahiro T. Nakamura},
	Date-Added = {2020-02-26 14:07:06 -0500},
	Date-Modified = {2020-02-26 14:07:13 -0500},
	Doi = {10.1103/PhysRevLett.80.1138},
	Journal = {Physical Review Letters},
	Number = {6},
	Pages = {1138--1141},
	Title = {Gravitational Lensing of Gravitational Waves from Inspiraling Binaries by a Point Mass Lens},
	Volume = {80},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevLett.80.1138}}

@article{amaro_2017,
	Author = {Pau Amaro-Seoane and Heather Audley and Stanislav Babak and John Baker and Enrico Barausse and Peter Bender and Emanuele Berti and Pierre Binetruy and Michael Born and Daniele Bortoluzzi and Jordan Camp and Chiara Caprini and Vitor Cardoso and Monica Colpi and John Conklin and Neil Cornish and Curt Cutler and Karsten Danzmann and Rita Dolesi and Luigi Ferraioli and Valerio Ferroni and Ewan Fitzsimons and Jonathan Gair and Lluis Gesa Bote and Domenico Giardini and Ferran Gibert and Catia Grimani and Hubert Halloin and Gerhard Heinzel and Thomas Hertog and Martin Hewitson and Kelly Holley-Bockelmann and Daniel Hollington and Mauro Hueller and Henri Inchauspe and Philippe Jetzer and Nikos Karnesis and Christian Killow and Antoine Klein and Bill Klipstein and Natalia Korsakova and Shane L Larson and Jeffrey Livas and Ivan Lloro and Nary Man and Davor Mance and Joseph Martino and Ignacio Mateos and Kirk McKenzie and Sean T McWilliams and Cole Miller and Guido Mueller and Germano Nardini and Gijs Nelemans and Miquel Nofrarias and Antoine Petiteau and Paolo Pivato and Eric Plagnol and Ed Porter and Jens Reiche and David Robertson and Norna Robertson and Elena Rossi and Giuliana Russano and Bernard Schutz and Alberto Sesana and David Shoemaker and Jacob Slutsky and Carlos F. Sopuerta and Tim Sumner and Nicola Tamanini and Ira Thorpe and Michael Troebs and Michele Vallisneri and Alberto Vecchio and Daniele Vetrugno and Stefano Vitale and Marta Volonteri and Gudrun Wanner and Harry Ward and Peter Wass and William Weber and John Ziemer and Peter Zweifel},
	Date-Added = {2020-02-26 14:01:22 -0500},
	Date-Modified = {2020-02-26 14:03:01 -0500},
	Journal = {arXiv:1702.00786},
	Title = {Laser Interferometer Space Antenna},
	Year = {2017}}

@article{Babak_2017,
	Author = {Stanislav Babak},
	Date-Added = {2020-02-26 13:58:03 -0500},
	Date-Modified = {2020-02-26 13:58:12 -0500},
	Doi = {10.1103/PhysRevD.95.103012},
	Journal = {Physical Review D},
	Number = {10},
	Title = {Science with the space-based interferometer LISA. V. Extreme mass-ratio inspirals},
	Volume = {95},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.95.103012}}

@article{Kocsis_2013,
	Author = {Kocsis, Bence},
	Date-Added = {2020-02-26 13:40:00 -0500},
	Date-Modified = {2020-02-26 13:40:00 -0500},
	Doi = {10.1088/0004-637x/763/2/122},
	Issn = {1538-4357},
	Journal = {The Astrophysical Journal},
	Month = {Jan},
	Number = {2},
	Pages = {122},
	Publisher = {IOP Publishing},
	Title = {HIGH-FREQUENCY GRAVITATIONAL WAVES FROM SUPERMASSIVE BLACK HOLES: PROSPECTS FOR LIGO-VIRGO DETECTIONS},
	Url = {http://dx.doi.org/10.1088/0004-637X/763/2/122},
	Volume = {763},
	Year = {2013},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/763/2/122},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/763/2/122}}

@article{dorazio_2019,
	Author = {D'Orazio, Daniel J. and Loeb, Abraham},
	Date-Added = {2020-02-26 12:12:47 -0500},
	Date-Modified = {2020-02-26 12:13:57 -0500},
	Journal = { arXiv:1910.02966},
	Title = {Repeated Gravitational Lensing of Gravitational Waves in Hierarchical Black Hole Triples},
	Year = {2019}}

@article{Yang_2019b,
	Author = {Yang, Y. and Bartos, I. and Gayathri, V. and Ford, K. E. S. and Haiman, Z. and Klimenko, S. and Kocsis, B. and M{\'a}rka, S. and M{\'a}rka, Z. and McKernan, B. and et al.},
	Date-Added = {2020-02-26 10:23:32 -0500},
	Date-Modified = {2020-02-26 10:23:40 -0500},
	Doi = {10.1103/physrevlett.123.181101},
	Issn = {1079-7114},
	Journal = {Physical Review Letters},
	Month = {Nov},
	Number = {18},
	Publisher = {American Physical Society (APS)},
	Title = {Hierarchical Black Hole Mergers in Active Galactic Nuclei},
	Url = {http://dx.doi.org/10.1103/PhysRevLett.123.181101},
	Volume = {123},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.123.181101},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevlett.123.181101}}

@article{Varma_2019,
	Author = {Varma, Vijay and Gerosa, Davide and Stein, Leo C. and H{\'e}bert, Fran{\c c}ois and Zhang, Hao},
	Date-Added = {2020-02-23 21:06:54 -0500},
	Date-Modified = {2020-02-23 21:06:54 -0500},
	Doi = {10.1103/physrevlett.122.011101},
	Issn = {1079-7114},
	Journal = {Physical Review Letters},
	Month = {Jan},
	Number = {1},
	Publisher = {American Physical Society (APS)},
	Title = {High-Accuracy Mass, Spin, and Recoil Predictions of Generic Black-Hole Merger Remnants},
	Url = {http://dx.doi.org/10.1103/PhysRevLett.122.011101},
	Volume = {122},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.122.011101},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevlett.122.011101}}

@article{Tichy_2008,
	Author = {Tichy, Wolfgang and Marronetti, Pedro},
	Date-Added = {2020-02-23 21:06:05 -0500},
	Date-Modified = {2020-02-23 21:06:05 -0500},
	Doi = {10.1103/physrevd.78.081501},
	Issn = {1550-2368},
	Journal = {Physical Review D},
	Month = {Oct},
	Number = {8},
	Publisher = {American Physical Society (APS)},
	Title = {Final mass and spin of black-hole mergers},
	Url = {http://dx.doi.org/10.1103/PhysRevD.78.081501},
	Volume = {78},
	Year = {2008},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.78.081501},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevd.78.081501}}

@article{Yang_2019a,
	Author = {Yang, Y. and Bartos, I. and Haiman, Z. and Kocsis, B. and M{\'a}rka, Z. and Stone, N. C. and M{\'a}rka, S.},
	Date-Added = {2020-02-22 17:17:18 -0500},
	Date-Modified = {2020-02-26 10:23:47 -0500},
	Doi = {10.3847/1538-4357/ab16e3},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {May},
	Number = {2},
	Pages = {122},
	Publisher = {American Astronomical Society},
	Title = {AGN Disks Harden the Mass Distribution of Stellar-mass Binary Black Hole Mergers},
	Url = {http://dx.doi.org/10.3847/1538-4357/ab16e3},
	Volume = {876},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/ab16e3}}

@article{Acernese_2014,
	Author = {Acernese, F and Agathos, M and Agatsuma, K and Aisa, D and Allemandou, N and Allocca, A and Amarni, J and Astone, P and Balestri, G and Ballardin, G and et al.},
	Date-Added = {2020-02-22 16:22:11 -0500},
	Date-Modified = {2020-02-22 16:22:11 -0500},
	Doi = {10.1088/0264-9381/32/2/024001},
	Issn = {1361-6382},
	Journal = {Classical and Quantum Gravity},
	Month = {Dec},
	Number = {2},
	Pages = {024001},
	Publisher = {IOP Publishing},
	Title = {Advanced Virgo: a second-generation interferometric gravitational wave detector},
	Url = {http://dx.doi.org/10.1088/0264-9381/32/2/024001},
	Volume = {32},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0264-9381/32/2/024001}}

@article{aasi_2015,
	Author = {Aasi, J and Abbott, B P and Abbott, R and Abbott, T and Abernathy, M R and Ackley, K and Adams, C and Adams, T and Addesso, P and et al.},
	Date-Added = {2020-02-22 16:21:14 -0500},
	Date-Modified = {2020-02-22 16:21:28 -0500},
	Doi = {10.1088/0264-9381/32/7/074001},
	Issn = {1361-6382},
	Journal = {Classical and Quantum Gravity},
	Month = {Mar},
	Number = {7},
	Pages = {074001},
	Publisher = {IOP Publishing},
	Title = {Advanced LIGO},
	Url = {http://dx.doi.org/10.1088/0264-9381/32/7/074001},
	Volume = {32},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0264-9381/32/7/074001}}

@article{Bonetti_2020,
	Author = {Bonetti, Matteo and Rasskazov, Alexander and Sesana, Alberto and Dotti, Massimo and Haardt, Francesco and Leigh, Nathan W C and Sedda, Manuel Arca and Fragione, Giacomo and Rossi, Elena},
	Date-Added = {2020-02-10 11:01:34 -0500},
	Date-Modified = {2020-02-24 20:43:26 -0500},
	Doi = {10.1093/mnrasl/slaa018},
	Issn = {1745-3933},
	Journal = {\mnrasL},
	Month = {Feb},
	Publisher = {Oxford University Press (OUP)},
	Title = {On the eccentricity evolution of massive black hole binaries in stellar backgrounds},
	Url = {http://dx.doi.org/10.1093/mnrasl/slaa018},
	Year = {2020},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnrasl/slaa018}}

@article{Moody_2019,
	Author = {Moody, Mackenzie S. L. and Shi, Ji-Ming and Stone, James M.},
	Date-Added = {2020-02-06 17:37:13 -0500},
	Date-Modified = {2020-02-24 20:41:24 -0500},
	Doi = {10.3847/1538-4357/ab09ee},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Apr},
	Number = {1},
	Pages = {66},
	Publisher = {American Astronomical Society},
	Title = {Hydrodynamic Torques in Circumbinary Accretion Disks},
	Url = {http://dx.doi.org/10.3847/1538-4357/ab09ee},
	Volume = {875},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/ab09ee}}

@article{Wang_2016,
	Author = {Wang, Long and Spurzem, Rainer and Aarseth, Sverre and Giersz, Mirek and Askar, Abbas and Berczik, Peter and Naab, Thorsten and Schadow, Riko and Kouwenhoven, M. B. N.},
	Date-Added = {2020-02-06 17:36:09 -0500},
	Date-Modified = {2020-02-24 20:44:48 -0500},
	Doi = {10.1093/mnras/stw274},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Feb},
	Number = {2},
	Pages = {1450--1465},
	Publisher = {Oxford University Press (OUP)},
	Title = {The dragon simulations: globular cluster evolution with a million stars},
	Url = {http://dx.doi.org/10.1093/mnras/stw274},
	Volume = {458},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw274}}

@article{Benacquista_2013,
	Author = {Benacquista, Matthew J. and Downing, Jonathan M. B.},
	Date-Added = {2020-02-06 17:33:55 -0500},
	Date-Modified = {2020-02-06 17:33:55 -0500},
	Doi = {10.12942/lrr-2013-4},
	Issn = {1433-8351},
	Journal = {Living Reviews in Relativity},
	Month = {Mar},
	Number = {1},
	Publisher = {Springer Science and Business Media LLC},
	Title = {Relativistic Binaries in Globular Clusters},
	Url = {http://dx.doi.org/10.12942/lrr-2013-4},
	Volume = {16},
	Year = {2013},
	Bdsk-Url-1 = {http://dx.doi.org/10.12942/lrr-2013-4}}

@article{de_Mink_2016,
	Author = {De Mink, S. E. and Mandel, I.},
	Date-Added = {2020-02-06 17:33:12 -0500},
	Date-Modified = {2020-02-24 20:46:14 -0500},
	Doi = {10.1093/mnras/stw1219},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {May},
	Number = {4},
	Pages = {3545--3553},
	Publisher = {Oxford University Press (OUP)},
	Title = {The chemically homogeneous evolutionary channel for binary black hole mergers: rates and properties of gravitational-wave events detectable by advanced LIGO},
	Url = {http://dx.doi.org/10.1093/mnras/stw1219},
	Volume = {460},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw1219}}

@article{Postnov_2014,
	Author = {Postnov, Konstantin A. and Yungelson, Lev R.},
	Date-Added = {2020-02-06 17:32:11 -0500},
	Date-Modified = {2020-02-06 17:32:11 -0500},
	Doi = {10.12942/lrr-2014-3},
	Issn = {1433-8351},
	Journal = {Living Reviews in Relativity},
	Month = {May},
	Number = {1},
	Publisher = {Springer Science and Business Media LLC},
	Title = {The Evolution of Compact Binary Star Systems},
	Url = {http://dx.doi.org/10.12942/lrr-2014-3},
	Volume = {17},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.12942/lrr-2014-3}}

@article{Belczynski_2010,
	Author = {Belczynski, Krzysztof and Bulik, Tomasz and Fryer, Chris L. and Ruiter, Ashley and Valsecchi, Francesca and Vink, Jorick S. and Hurley, Jarrod R.},
	Date-Added = {2020-02-06 17:31:53 -0500},
	Date-Modified = {2020-02-24 20:41:04 -0500},
	Doi = {10.1088/0004-637x/714/2/1217},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Apr},
	Number = {2},
	Pages = {1217--1226},
	Publisher = {IOP Publishing},
	Title = {ON THE MAXIMUM MASS OF STELLAR BLACK HOLES},
	Url = {http://dx.doi.org/10.1088/0004-637X/714/2/1217},
	Volume = {714},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/2/1217},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/714/2/1217}}

@article{Lin_1986,
	Author = {Lin, D. N. C. and Papaloizou, John},
	Date-Added = {2020-02-06 12:17:10 -0500},
	Date-Modified = {2020-02-24 20:41:18 -0500},
	Doi = {10.1086/164653},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Oct},
	Pages = {846},
	Publisher = {IOP Publishing},
	Title = {On the tidal interaction between protoplanets and the protoplanetary disk. III - Orbital migration of protoplanets},
	Url = {http://dx.doi.org/10.1086/164653},
	Volume = {309},
	Year = {1986},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/164653}}

@book{1987_binney,
	Author = {Binney, James anbd Tremaine, Scott},
	Date-Added = {2020-02-06 12:13:49 -0500},
	Date-Modified = {2020-02-06 12:14:59 -0500},
	Publisher = {Princeton University Press},
	Title = {Galactic Dynamics},
	Year = {1987}}

@article{Masset_2017,
	Author = {Masset, Fr{\'e}d{\'e}ric S.},
	Date-Added = {2020-02-06 12:10:19 -0500},
	Date-Modified = {2020-02-24 20:44:18 -0500},
	Doi = {10.1093/mnras/stx2271},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Sep},
	Number = {4},
	Pages = {4204--4219},
	Publisher = {Oxford University Press (OUP)},
	Title = {Coorbital thermal torques on low-mass protoplanets},
	Url = {http://dx.doi.org/10.1093/mnras/stx2271},
	Volume = {472},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx2271}}

@article{Eklund_2017,
	Author = {Eklund, Henrik and Masset, Fr{\'e}d{\'e}ric S.},
	Date-Added = {2020-02-06 12:09:49 -0500},
	Date-Modified = {2020-02-24 20:43:59 -0500},
	Doi = {10.1093/mnras/stx856},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Apr},
	Number = {1},
	Pages = {206--217},
	Publisher = {Oxford University Press (OUP)},
	Title = {Evolution of eccentricity and inclination of hot protoplanets embedded in radiative discs},
	Url = {http://dx.doi.org/10.1093/mnras/stx856},
	Volume = {469},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx856}}

@article{Benitez_2015,
	Author = {Ben{\'\i}tez-Llambay, Pablo and Masset, Fr{\'e}d{\'e}ric and Koenigsberger, Gloria and Szul{\'a}gyi, Judit},
	Date-Added = {2020-02-06 12:08:58 -0500},
	Date-Modified = {2020-02-06 12:09:08 -0500},
	Doi = {10.1038/nature14277},
	Issn = {1476-4687},
	Journal = {Nature},
	Month = {Apr},
	Number = {7545},
	Pages = {63--65},
	Publisher = {Springer Science and Business Media LLC},
	Title = {Planet heating prevents inward migration of planetary cores},
	Url = {http://dx.doi.org/10.1038/nature14277},
	Volume = {520},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature14277}}

@article{Comins_2016,
	Author = {Comins, Megan L. and Romanova, Marina M. and Koldoba, Alexander V. and Ustyugova, Galina V. and Blinova, Alisa A. and Lovelace, Richard V. E.},
	Date-Added = {2020-02-06 12:07:48 -0500},
	Date-Modified = {2020-02-24 20:43:45 -0500},
	Doi = {10.1093/mnras/stw843},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Apr},
	Number = {4},
	Pages = {3482--3497},
	Publisher = {Oxford University Press (OUP)},
	Title = {The effects of a magnetic field on planetary migration in laminar and turbulent discs},
	Url = {http://dx.doi.org/10.1093/mnras/stw843},
	Volume = {459},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw843}}

@article{Guilet_2013,
	Author = {Guilet, J{\'e}r{\^o}me and Baruteau, Cl{\'e}ment and Papaloizou, John C. B.},
	Date-Added = {2020-02-06 12:06:54 -0500},
	Date-Modified = {2020-02-24 20:44:05 -0500},
	Doi = {10.1093/mnras/sts720},
	Issn = {0035-8711},
	Journal = {\mnras},
	Month = {Feb},
	Number = {3},
	Pages = {1764--1783},
	Publisher = {Oxford University Press (OUP)},
	Title = {Type I planet migration in weakly magnetized laminar discs},
	Url = {http://dx.doi.org/10.1093/mnras/sts720},
	Volume = {430},
	Year = {2013},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts720}}

@article{Uribe_2011,
	Author = {Uribe, A. L. and Klahr, H. and Flock, M. and Henning, Th.},
	Date-Added = {2020-02-06 12:06:16 -0500},
	Date-Modified = {2020-02-24 20:41:35 -0500},
	Doi = {10.1088/0004-637x/736/2/85},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Jul},
	Number = {2},
	Pages = {85},
	Publisher = {IOP Publishing},
	Title = {THREE-DIMENSIONAL MAGNETOHYDRODYNAMIC SIMULATIONS OF PLANET MIGRATION IN TURBULENT STRATIFIED DISKS},
	Url = {http://dx.doi.org/10.1088/0004-637X/736/2/85},
	Volume = {736},
	Year = {2011},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/736/2/85},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/736/2/85}}

@article{Uribe_2015,
	Author = {Uribe, Ana and Bans, Alissa and K{\"o}nigl, Arieh},
	Date-Added = {2020-02-06 12:05:21 -0500},
	Date-Modified = {2020-02-24 20:41:41 -0500},
	Doi = {10.1088/0004-637x/802/1/54},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Mar},
	Number = {1},
	Pages = {54},
	Publisher = {IOP Publishing},
	Title = {TYPE I PLANET MIGRATION IN A MAGNETIZED DISK. I. EFFECT OF LARGE-SCALE VERTICAL AND AZIMUTHAL FIELD COMPONENTS},
	Url = {http://dx.doi.org/10.1088/0004-637X/802/1/54},
	Volume = {802},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/802/1/54},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/802/1/54}}

@article{Nelson_2004,
	Author = {Nelson, Richard P. and Papaloizou, John C. B.},
	Date-Added = {2020-02-06 12:04:26 -0500},
	Date-Modified = {2020-02-24 20:44:25 -0500},
	Doi = {10.1111/j.1365-2966.2004.07406.x},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {May},
	Number = {3},
	Pages = {849--864},
	Publisher = {Oxford University Press (OUP)},
	Title = {The interaction of giant planets with a disc with MHD turbulence - IV. Migration rates of embedded protoplanets},
	Url = {http://dx.doi.org/10.1111/j.1365-2966.2004.07406.x},
	Volume = {350},
	Year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07406.x}}

@article{Pierens_2015,
	Author = {Pierens, A.},
	Date-Added = {2020-02-06 12:03:18 -0500},
	Date-Modified = {2020-02-24 20:44:43 -0500},
	Doi = {10.1093/mnras/stv2024},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Oct},
	Number = {2},
	Pages = {2003--2014},
	Publisher = {Oxford University Press (OUP)},
	Title = {Fast migration of low-mass planets in radiative discs},
	Url = {http://dx.doi.org/10.1093/mnras/stv2024},
	Volume = {454},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv2024}}

@article{Paardekooper_2014,
	Author = {Paardekooper, S.-J.},
	Date-Added = {2020-02-06 12:02:55 -0500},
	Date-Modified = {2020-02-24 20:44:36 -0500},
	Doi = {10.1093/mnras/stu1542},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Sep},
	Number = {3},
	Pages = {2031--2042},
	Publisher = {Oxford University Press (OUP)},
	Title = {Dynamical corotation torques on low-mass planets},
	Url = {http://dx.doi.org/10.1093/mnras/stu1542},
	Volume = {444},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu1542}}

@article{Coleman_2014,
	Author = {Coleman, Gavin A. L. and Nelson, Richard P.},
	Date-Added = {2020-02-06 12:02:11 -0500},
	Date-Modified = {2020-02-24 20:43:34 -0500},
	Doi = {10.1093/mnras/stu1715},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Sep},
	Number = {1},
	Pages = {479--499},
	Publisher = {Oxford University Press (OUP)},
	Title = {On the formation of planetary systems via oligarchic growth in thermally evolving viscous discs},
	Url = {http://dx.doi.org/10.1093/mnras/stu1715},
	Volume = {445},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu1715}}

@article{Paardekooper_2011,
	Author = {Paardekooper, S.-J. and Baruteau, C. and Kley, W.},
	Date-Added = {2020-02-06 12:01:08 -0500},
	Date-Modified = {2020-02-24 20:44:31 -0500},
	Doi = {10.1111/j.1365-2966.2010.17442.x},
	Issn = {0035-8711},
	Journal = {\mnras},
	Month = {Sep},
	Number = {1},
	Pages = {293--303},
	Publisher = {Oxford University Press (OUP)},
	Title = {A torque formula for non-isothermal Type I planetary migration - II. Effects of diffusion},
	Url = {http://dx.doi.org/10.1111/j.1365-2966.2010.17442.x},
	Volume = {410},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17442.x}}

@article{mckernan19,
	Author = {{McKernan}, B. and {Ford}, K.~E.~S. and O'Shaughnessy, Richard and Wysoki, D.},
	Date-Added = {2020-02-06 11:58:17 -0500},
	Date-Modified = {2020-02-24 20:46:52 -0500},
	Journal = {arXiv:1907.04356},
	Title = {Monte-Carlo simulations of black hole mergers in AGN disks: Low χeff mergers and predictions for LIGO},
	Year = {2019}}

@article{tagawa_2019,
	Author = {Tagawa, Hiromichi and {Haiman}, Z. and {Kocsis}, B.},
	Date-Added = {2020-02-06 11:54:20 -0500},
	Date-Modified = {2020-02-06 11:59:33 -0500},
	Journal = {arXiv:1912.08218},
	Title = {Formation and Evolution of Compact Object Binaries in AGN Disks},
	Year = {2019}}

@article{secunda,
	Author = {Secunda, Amy and Bellovary, Jillian and Low, Mordecai-Mark Mac and Ford, K. E. Saavik and McKernan, Barry and Leigh, Nathan W. C. and Lyra, Wladimir and S{\'a}ndor, Zsolt},
	Date-Added = {2020-02-06 11:52:59 -0500},
	Date-Modified = {2020-02-24 20:41:30 -0500},
	Doi = {10.3847/1538-4357/ab20ca},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Jun},
	Number = {2},
	Pages = {85},
	Publisher = {American Astronomical Society},
	Title = {Orbital Migration of Interacting Stellar Mass Black Holes in Disks around Supermassive Black Holes},
	Url = {http://dx.doi.org/10.3847/1538-4357/ab20ca},
	Volume = {878},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/ab20ca}}

@article{belczynski,
	Author = {Belczynski, Krzysztof and Holz, Daniel E. and Bulik, Tomasz and O'Shaughnessy, Richard},
	Date-Added = {2020-02-06 11:52:13 -0500},
	Date-Modified = {2020-02-06 11:52:22 -0500},
	Doi = {10.1038/nature18322},
	Issn = {1476-4687},
	Journal = {Nature},
	Month = {Jun},
	Number = {7608},
	Pages = {512--515},
	Publisher = {Springer Science and Business Media LLC},
	Title = {The first gravitational-wave source from the isolated evolution of two stars in the 40--100 solar mass range},
	Url = {http://dx.doi.org/10.1038/nature18322},
	Volume = {534},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature18322}}

@article{Abbott_2019,
	Author = {Abbott, B. P. and Abbott, R. and Abbott, T. D. and Abraham, S. and Acernese, F. and Ackley, K. and Adams, C. and Adhikari, R. X. and Adya, V. B. and Affeldt, C. and et al.},
	Date-Added = {2020-02-06 11:50:52 -0500},
	Date-Modified = {2020-02-06 11:50:52 -0500},
	Doi = {10.1103/physrevx.9.031040},
	Issn = {2160-3308},
	Journal = {Physical Review X},
	Month = {Sep},
	Number = {3},
	Publisher = {American Physical Society (APS)},
	Title = {GWTC-1: A Gravitational-Wave Transient Catalog of Compact Binary Mergers Observed by LIGO and Virgo during the First and Second Observing Runs},
	Url = {http://dx.doi.org/10.1103/PhysRevX.9.031040},
	Volume = {9},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevX.9.031040},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevx.9.031040}}

@article{Dittkrist_2014,
	Author = {Dittkrist, K.-M. and Mordasini, C. and Klahr, H. and Alibert, Y. and Henning, T.},
	Date-Added = {2020-01-23 15:07:21 -0500},
	Date-Modified = {2020-02-24 20:45:25 -0500},
	Doi = {10.1051/0004-6361/201322506},
	Issn = {1432-0746},
	Journal = {\aap},
	Month = {Jul},
	Pages = {A121},
	Publisher = {EDP Sciences},
	Title = {Impacts of planet migration models on planetary populations},
	Url = {http://dx.doi.org/10.1051/0004-6361/201322506},
	Volume = {567},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201322506}}

@article{Coleman_2016,
	Author = {Coleman, Gavin A. L. and Nelson, Richard P.},
	Date-Added = {2020-01-23 15:06:41 -0500},
	Date-Modified = {2020-02-24 20:43:40 -0500},
	Doi = {10.1093/mnras/stw149},
	Issn = {1365-2966},
	Journal = {\mnras},
	Month = {Feb},
	Number = {3},
	Pages = {2480--2500},
	Publisher = {Oxford University Press (OUP)},
	Title = {On the formation of compact planetary systems via concurrent core accretion and migration},
	Url = {http://dx.doi.org/10.1093/mnras/stw149},
	Volume = {457},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw149}}

@article{Hellary_2011,
	Author = {Hellary, Phil and Nelson, Richard P.},
	Date-Added = {2020-01-23 15:05:22 -0500},
	Date-Modified = {2020-02-24 20:44:12 -0500},
	Doi = {10.1111/j.1365-2966.2011.19815.x},
	Issn = {0035-8711},
	Journal = {\mnras},
	Month = {Dec},
	Number = {4},
	Pages = {2737--2757},
	Publisher = {Oxford University Press (OUP)},
	Title = {Global models of planetary system formation in radiatively-inefficient protoplanetary discs},
	Url = {http://dx.doi.org/10.1111/j.1365-2966.2011.19815.x},
	Volume = {419},
	Year = {2011},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19815.x}}

@article{jiang_stone,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170902845J},
	Archiveprefix = {arXiv},
	Author = {{Jiang}, Y.-F. and {Stone}, J. and {Davis}, S.~W.},
	Date-Added = {2018-07-06 15:09:44 +0000},
	Date-Modified = {2018-07-06 15:09:54 +0000},
	Eprint = {1709.02845},
	Journal = {ArXiv e-prints},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = sep,
	Primaryclass = {astro-ph.HE},
	Title = {{Super-Eddington Accretion Disks around Supermassive black Holes}},
	Year = 2017}

@article{bahcall_wolf,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...209..214B},
	Author = {{Bahcall}, J.~N. and {Wolf}, R.~A.},
	Date-Added = {2018-07-02 16:09:46 +0000},
	Date-Modified = {2018-07-02 16:09:56 +0000},
	Doi = {10.1086/154711},
	Journal = {\apj},
	Keywords = {Black Holes (Astronomy), Distribution Functions, Globular Clusters, Gravitational Effects, Star Distribution, Stellar Motions, Anisotropy, Density (Number/Volume), Flow Velocity, Gravitational Fields, Stellar Mass, Time Dependence, Velocity Distribution, X Ray Sources},
	Month = oct,
	Pages = {214-232},
	Title = {{Star distribution around a massive black hole in a globular cluster}},
	Volume = 209,
	Year = 1976,
	Bdsk-Url-1 = {https://doi.org/10.1086/154711}}

@article{schawinski,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451.2517S},
	Archiveprefix = {arXiv},
	Author = {{Schawinski}, K. and {Koss}, M. and {Berney}, S. and {Sartori}, L.~F.},
	Date-Added = {2018-06-20 16:23:09 +0000},
	Date-Modified = {2018-06-20 16:23:16 +0000},
	Doi = {10.1093/mnras/stv1136},
	Eprint = {1505.06733},
	Journal = {\mnras},
	Keywords = {galaxies: active, quasars: general, galaxies: Seyfert},
	Month = aug,
	Pages = {2517-2523},
	Title = {{Active galactic nuclei flicker: an observational estimate of the duration of black hole growth phases of {\tilde}10$^{5}$ yr}},
	Volume = 451,
	Year = 2015,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stv1136}}

@article{king_nixon,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.453L..46K},
	Archiveprefix = {arXiv},
	Author = {{King}, A. and {Nixon}, C.},
	Date-Added = {2018-06-20 16:22:22 +0000},
	Date-Modified = {2018-06-20 16:22:33 +0000},
	Doi = {10.1093/mnrasl/slv098},
	Eprint = {1507.05960},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, galaxies: active, quasars: supermassive black holes, galaxies: Seyfert, X-rays: galaxies},
	Month = oct,
	Pages = {L46-L47},
	Primaryclass = {astro-ph.HE},
	Title = {{AGN flickering and chaotic accretion}},
	Volume = 453,
	Year = 2015,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnrasl/slv098}}

@article{haehnelt,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.263..168H},
	Author = {{Haehnelt}, M.~G. and {Rees}, M.~J.},
	Date-Added = {2018-06-20 16:21:05 +0000},
	Date-Modified = {2018-06-20 16:21:16 +0000},
	Doi = {10.1093/mnras/263.1.168},
	Journal = {\mnras},
	Keywords = {Active Galactic Nuclei, Black Holes (Astronomy), Galactic Evolution, Quasars, Red Shift, Astronomical Models, Dark Matter, Galactic Structure, Halos, Stellar Luminosity},
	Month = jul,
	Pages = {168-178},
	Title = {{The formation of nuclei in newly formed galaxies and the evolution of the quasar population}},
	Volume = 263,
	Year = 1993,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/263.1.168}}

@article{Cresswell_2006,
	Author = {Cresswell, P. and Nelson, R. P.},
	Date-Added = {2018-06-16 18:31:34 +0000},
	Date-Modified = {2018-07-02 16:17:54 +0000},
	Doi = {10.1051/0004-6361:20054551},
	Issn = {1432-0746},
	Journal = {\aap},
	Month = {Apr},
	Number = {2},
	Pages = {833--853},
	Publisher = {EDP Sciences},
	Title = {On the evolution of multiple protoplanets embedded in a protostellar disc},
	Url = {http://dx.doi.org/10.1051/0004-6361:20054551},
	Volume = {450},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054551}}

@article{baruteau2011,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...726...28B},
	Author = {{Baruteau}, C. and {Cuadra}, J. and {Lin}, D.~N.~C.},
	Date-Added = {2018-06-04 18:21:40 +0000},
	Date-Modified = {2018-06-04 18:21:51 +0000},
	Doi = {10.1088/0004-637X/726/1/28},
	Eid = {28},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, binaries: general, Galaxy: center, hydrodynamics, methods: numerical},
	Month = jan,
	Pages = {28},
	Title = {{Binaries Migrating in a Gaseous Disk: Where are the Galactic Center Binaries?}},
	Volume = 726,
	Year = 2011,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/726/1/28}}

@article{mckernan18,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170207818M},
	Archiveprefix = {arXiv},
	Author = {{McKernan}, B. and {Ford}, K.~E.~S. and {Bellovary}, J. and {Leigh}, N.~W.~C. and {Haiman}, Z. and {Kocsis}, B. and {Lyra}, W. and {MacLow}, M.-M. and {Metzger}, B. and {O'Dowd}, M. and {Endlich}, S. and {Rosen}, D.~J.},
	Date-Added = {2018-05-08 17:47:19 +0000},
	Date-Modified = {2018-05-08 17:47:30 +0000},
	Eprint = {1702.07818},
	Journal = {ArXiv e-prints},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, General Relativity and Quantum Cosmology},
	Month = feb,
	Primaryclass = {astro-ph.HE},
	Title = {{On stellar-mass black hole mergers in AGN disks detectable with LIGO}},
	Year = 2017}

@article{mckernan14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441..900M},
	Archiveprefix = {arXiv},
	Author = {{McKernan}, B. and {Ford}, K.~E.~S. and {Kocsis}, B. and {Lyra}, W. and {Winter}, L.~M.},
	Date-Added = {2018-05-07 19:04:55 +0000},
	Date-Modified = {2018-05-07 19:05:02 +0000},
	Doi = {10.1093/mnras/stu553},
	Eprint = {1403.6433},
	Journal = {\mnras},
	Keywords = {accretion accretion discs, planets and satellites: formation, planet-disc interactions, protoplanetary discs, galaxies: active, galaxies: Seyfert},
	Month = jun,
	Pages = {900-909},
	Title = {{Intermediate-mass black holes in AGN discs - II. Model predictions and observational constraints}},
	Volume = 441,
	Year = 2014,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stu553}}

@article{fryer,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...749...91F},
	Archiveprefix = {arXiv},
	Author = {{Fryer}, C.~L. and {Belczynski}, K. and {Wiktorowicz}, G. and {Dominik}, M. and {Kalogera}, V. and {Holz}, D.~E.},
	Date-Added = {2018-04-30 18:56:42 +0000},
	Date-Modified = {2018-04-30 18:56:50 +0000},
	Doi = {10.1088/0004-637X/749/1/91},
	Eid = {91},
	Eprint = {1110.1726},
	Journal = {\apj},
	Keywords = {black hole physics, stars: neutron, supernovae: general},
	Month = apr,
	Pages = {91},
	Primaryclass = {astro-ph.SR},
	Title = {{Compact Remnant Mass Function: Dependence on the Explosion Mechanism and Metallicity}},
	Volume = 749,
	Year = 2012,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/749/1/91}}

@article{peters,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1964PhRv..136.1224P},
	Author = {{Peters}, P.~C.},
	Date-Added = {2018-04-25 18:27:47 +0000},
	Date-Modified = {2018-04-25 18:27:55 +0000},
	Doi = {10.1103/PhysRev.136.B1224},
	Journal = {Physical Review},
	Month = nov,
	Pages = {1224-1232},
	Title = {{Gravitational Radiation and the Motion of Two Point Masses}},
	Volume = 136,
	Year = 1964,
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRev.136.B1224}}

@article{davis,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713...52D},
	Archiveprefix = {arXiv},
	Author = {{Davis}, S.~W. and {Stone}, J.~M. and {Pessah}, M.~E.},
	Date-Added = {2018-04-23 19:45:57 +0000},
	Date-Modified = {2018-04-23 19:46:05 +0000},
	Doi = {10.1088/0004-637X/713/1/52},
	Eprint = {0909.1570},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, hydrodynamics, methods: numerical},
	Month = apr,
	Pages = {52-65},
	Primaryclass = {astro-ph.HE},
	Title = {{Sustained Magnetorotational Turbulence in Local Simulations of Stratified Disks with Zero Net Magnetic Flux}},
	Volume = 713,
	Year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/713/1/52}}

@article{Hailey_2018,
	Author = {Hailey, Charles J. and Mori, Kaya and Bauer, Franz E. and Berkowitz, Michael E. and Hong, Jaesub and Hord, Benjamin J.},
	Date-Added = {2018-04-23 19:30:51 +0000},
	Date-Modified = {2018-04-23 19:30:51 +0000},
	Doi = {10.1038/nature25029},
	Issn = {1476-4687},
	Journal = {Nature},
	Month = {Apr},
	Number = {7699},
	Pages = {70--73},
	Publisher = {Springer Nature},
	Title = {A density cusp of quiescent X-ray binaries in the central parsec of the Galaxy},
	Url = {http://dx.doi.org/10.1038/nature25029},
	Volume = {556},
	Year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature25029}}

@article{leigh2016,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463.1605L},
	Archiveprefix = {arXiv},
	Author = {{Leigh}, N.~W.~C. and {Antonini}, F. and {Stone}, N.~C. and {Shara}, M.~M. and {Merritt}, D.},
	Date-Added = {2018-04-23 19:17:10 +0000},
	Date-Modified = {2018-04-23 19:17:23 +0000},
	Doi = {10.1093/mnras/stw2018},
	Eprint = {1608.02944},
	Journal = {\mnras},
	Keywords = {galaxies: nuclei, blue stragglers, galaxies: photometry, stars: kinematics and dynamics, stars: black holes, Galaxy: centre},
	Month = dec,
	Pages = {1605-1623},
	Title = {{On the origins of enigmatic stellar populations in Local Group galactic nuclei}},
	Volume = 463,
	Year = 2016,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stw2018}}

@article{davies,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301..745D},
	Author = {{Davies}, M.~B. and {Blackwell}, R. and {Bailey}, V.~C. and {Sigurdsson}, S.},
	Date-Added = {2018-04-23 19:09:20 +0000},
	Date-Modified = {2018-04-23 19:09:28 +0000},
	Doi = {10.1046/j.1365-8711.1998.02027.x},
	Journal = {\mnras},
	Keywords = {CELESTIAL MECHANICS, STELLAR DYNAMICS, BINARIES: GENERAL, GALAXY: CENTRE},
	Month = dec,
	Pages = {745-753},
	Title = {{The destructive effects of binary encounters on red giants in the Galactic Centre}},
	Volume = 301,
	Year = 1998,
	Bdsk-Url-1 = {https://doi.org/10.1046/j.1365-8711.1998.02027.x}}

@article{leigh,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.474.5672L},
	Archiveprefix = {arXiv},
	Author = {{Leigh}, N.~W.~C. and {Geller}, A.~M. and {McKernan}, B. and {Ford}, K.~E.~S. and {Mac Low}, M.-M. and {Bellovary}, J. and {Haiman}, Z. and {Lyra}, W. and {Samsing}, J. and {O'Dowd}, M. and {Kocsis}, B. and {Endlich}, S.},
	Date-Added = {2018-04-23 17:28:50 +0000},
	Date-Modified = {2018-04-23 17:29:13 +0000},
	Doi = {10.1093/mnras/stx3134},
	Eprint = {1711.10494},
	Journal = {\mnras},
	Keywords = {black hole physics, gravitational waves, scattering, binaries: general, galaxies: active, galaxies: nuclei},
	Month = mar,
	Pages = {5672-5683},
	Title = {{On the rate of black hole binary mergers in galactic nuclei due to dynamical hardening}},
	Volume = 474,
	Year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stx3134}}

@article{kroupa,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002Sci...295...82K},
	Author = {{Kroupa}, P.},
	Date-Added = {2018-04-18 03:33:59 +0000},
	Date-Modified = {2018-04-18 03:34:12 +0000},
	Doi = {10.1126/science.1067524},
	Eprint = {astro-ph/0201098},
	Journal = {Science},
	Month = jan,
	Pages = {82-91},
	Title = {{The Initial Mass Function of Stars: Evidence for Uniformity in Variable Systems}},
	Volume = 295,
	Year = 2002,
	Bdsk-Url-1 = {https://doi.org/10.1126/science.1067524}}

@article{antonini,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794..106A},
	Archiveprefix = {arXiv},
	Author = {{Antonini}, F.},
	Date-Added = {2018-04-18 03:29:50 +0000},
	Date-Modified = {2018-04-18 03:30:01 +0000},
	Doi = {10.1088/0004-637X/794/2/106},
	Eid = {106},
	Eprint = {1402.4865},
	Journal = {\apj},
	Keywords = {galaxies: nuclei, Galaxy: center, Galaxy: formation, stars: black holes, stars: kinematics and dynamics},
	Month = oct,
	Pages = {106},
	Title = {{On the Distribution of Stellar Remnants around Massive Black Holes: Slow Mass Segregation, Star Cluster Inspirals, and Correlated Orbits}},
	Volume = 794,
	Year = 2014,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/794/2/106}}

@article{sandor,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...728L...9S},
	Archiveprefix = {arXiv},
	Author = {{S{\'a}ndor}, Z. and {Lyra}, W. and {Dullemond}, C.~P.},
	Date-Added = {2018-04-18 03:23:34 +0000},
	Date-Modified = {2018-04-18 03:23:48 +0000},
	Doi = {10.1088/2041-8205/728/1/L9},
	Eid = {L9},
	Eprint = {1101.0942},
	Journal = {\apjl},
	Keywords = {methods: numerical, planet-disk interactions, planets and satellites: formation, protoplanetary disks},
	Month = feb,
	Pages = {L9},
	Primaryclass = {astro-ph.EP},
	Title = {{Formation of Planetary Cores at Type I Migration Traps}},
	Volume = 728,
	Year = 2011,
	Bdsk-Url-1 = {https://doi.org/10.1088/2041-8205/728/1/L9}}

@article{cresswell_nelson,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..677C},
	Archiveprefix = {arXiv},
	Author = {{Cresswell}, P. and {Nelson}, R.~P.},
	Date-Added = {2018-04-18 03:22:08 +0000},
	Date-Modified = {2018-04-18 03:22:23 +0000},
	Doi = {10.1051/0004-6361:20079178},
	Eprint = {0811.4322},
	Journal = {\aap},
	Keywords = {stars: planetary systems: formation, stars: planetary systems: protoplanetary disks, stars: planetary systems},
	Month = may,
	Pages = {677-690},
	Title = {{Three-dimensional simulations of multiple protoplanets embedded in a protostellar disc}},
	Volume = 482,
	Year = 2008,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361:20079178}}

@article{tanaka_ward,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...602..388T},
	Author = {{Tanaka}, H. and {Ward}, W.~R.},
	Date-Added = {2018-04-18 03:21:00 +0000},
	Date-Modified = {2018-04-18 03:21:09 +0000},
	Doi = {10.1086/380992},
	Journal = {\apj},
	Keywords = {Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks, Solar System: Formation, Waves},
	Month = feb,
	Pages = {388-395},
	Title = {{Three-dimensional Interaction between a Planet and an Isothermal Gaseous Disk. II. Eccentricity Waves and Bending Waves}},
	Volume = 602,
	Year = 2004,
	Bdsk-Url-1 = {https://doi.org/10.1086/380992}}

@article{baruteau_lin,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...709..759B},
	Archiveprefix = {arXiv},
	Author = {{Baruteau}, C. and {Lin}, D.~N.~C.},
	Date-Added = {2018-04-18 03:19:01 +0000},
	Date-Modified = {2018-04-18 03:19:13 +0000},
	Doi = {10.1088/0004-637X/709/2/759},
	Eprint = {0912.0964},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, hydrodynamics, methods: numerical, planetary systems: formation, planetary systems: protoplanetary disks, turbulence},
	Month = feb,
	Pages = {759-773},
	Primaryclass = {astro-ph.EP},
	Title = {{Protoplanetary Migration in Turbulent Isothermal Disks}},
	Volume = 709,
	Year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/709/2/759}}

@article{ogihara,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Icar..188..522O},
	Author = {{Ogihara}, M. and {Ida}, S. and {Morbidelli}, A.},
	Date-Added = {2018-04-18 03:16:13 +0000},
	Date-Modified = {2018-04-18 03:17:54 +0000},
	Doi = {10.1016/j.icarus.2006.12.006},
	Eprint = {astro-ph/0612619},
	Journal = {\icarus},
	Month = jun,
	Pages = {522-534},
	Title = {{Accretion of terrestrial planets from oligarchs in a turbulent disk}},
	Volume = 188,
	Year = 2007,
	Bdsk-Url-1 = {https://doi.org/10.1016/j.icarus.2006.12.006}}

@article{Laughlin_1994,
	Author = {Laughlin, Gregory and Bodenheimer, Peter},
	Date-Added = {2018-04-18 03:15:14 +0000},
	Date-Modified = {2020-02-24 20:41:12 -0500},
	Doi = {10.1086/174909},
	Issn = {1538-4357},
	Journal = {\apj},
	Month = {Nov},
	Pages = {335},
	Publisher = {IOP Publishing},
	Title = {Nonaxisymmetric evolution in protostellar disks},
	Url = {http://dx.doi.org/10.1086/174909},
	Volume = {436},
	Year = {1994},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/174909}}

@article{kley_crida,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487L...9K},
	Archiveprefix = {arXiv},
	Author = {{Kley}, W. and {Crida}, A.},
	Date-Added = {2018-04-18 03:07:38 +0000},
	Date-Modified = {2018-04-18 03:07:52 +0000},
	Doi = {10.1051/0004-6361:200810033},
	Eprint = {0806.2990},
	Journal = {\aap},
	Keywords = {stars: planetary systems: formation, accretion, accretion disks},
	Month = aug,
	Pages = {L9-L12},
	Title = {{Migration of protoplanets in radiative discs}},
	Volume = 487,
	Year = 2008,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361:200810033}}

@article{hubeny,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...351..632H},
	Author = {{Hubeny}, I.},
	Date-Added = {2018-04-18 03:03:59 +0000},
	Date-Modified = {2018-04-18 03:04:06 +0000},
	Doi = {10.1086/168501},
	Journal = {\apj},
	Keywords = {Accretion Disks, Astronomical Models, Gray Gas, Stellar Atmospheres, Stellar Mass Accretion, Hydrostatics, Irradiation, Optical Thickness, Thermodynamic Equilibrium, Vertical Distribution, Viscous Damping},
	Month = mar,
	Pages = {632-641},
	Title = {{Vertical structure of accretion disks - A simplified analytical model}},
	Volume = 351,
	Year = 1990,
	Bdsk-Url-1 = {https://doi.org/10.1086/168501}}

@article{alexander_ferguson,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...437..879A},
	Author = {{Alexander}, D.~R. and {Ferguson}, J.~W.},
	Date-Added = {2018-04-18 02:59:58 +0000},
	Date-Modified = {2018-04-18 03:01:02 +0000},
	Doi = {10.1086/175039},
	Journal = {\apj},
	Keywords = {Cosmic Dust, Emission Spectra, Low Temperature, Molecular Spectra, Opacity, Plancks Constant, Radiative Transfer, Absorption Spectra, Equations Of State, Numerical Analysis, Rayleigh Scattering, Temperature Distribution, Triatomic Molecules},
	Month = dec,
	Pages = {879-891},
	Title = {{Low-temperature Rosseland opacities}},
	Volume = 437,
	Year = 1994,
	Bdsk-Url-1 = {https://doi.org/10.1086/175039}}

@article{iglesias_rogers,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..943I},
	Author = {{Iglesias}, C.~A. and {Rogers}, F.~J.},
	Date-Added = {2018-04-18 02:58:08 +0000},
	Date-Modified = {2018-04-18 02:58:19 +0000},
	Doi = {10.1086/177381},
	Journal = {\apj},
	Keywords = {ATOMIC DATA, ATOMIC PROCESSES, STARS: INTERIORS},
	Month = jun,
	Pages = {943},
	Title = {{Updated Opal Opacities}},
	Volume = 464,
	Year = 1996,
	Bdsk-Url-1 = {https://doi.org/10.1086/177381}}

@inproceedings{shakura_sunyaev,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1973IAUS...55..155S},
	Author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
	Booktitle = {X- and Gamma-Ray Astronomy},
	Date-Added = {2018-04-18 02:56:40 +0000},
	Date-Modified = {2018-04-18 02:56:53 +0000},
	Editor = {{Bradt}, H. and {Giacconi}, R.},
	Pages = {155},
	Series = {IAU Symposium},
	Title = {{Black Holes in Binary Systems: Observational Appearances}},
	Volume = 55,
	Year = 1973}

@article{thompson,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630..167T},
	Author = {{Thompson}, T.~A. and {Quataert}, E. and {Murray}, N.},
	Date-Added = {2018-04-18 02:53:29 +0000},
	Date-Modified = {2018-04-18 02:53:40 +0000},
	Doi = {10.1086/431923},
	Eprint = {astro-ph/0503027},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Galaxies: Formation, Galaxies: General, Galaxies: Starburst, Galaxy: Center, Galaxies: Quasars: General},
	Month = sep,
	Pages = {167-185},
	Title = {{Radiation Pressure-supported Starburst Disks and Active Galactic Nucleus Fueling}},
	Volume = 630,
	Year = 2005,
	Bdsk-Url-1 = {https://doi.org/10.1086/431923}}

@article{mckernan2012,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425..460M},
	Archiveprefix = {arXiv},
	Author = {{McKernan}, B. and {Ford}, K.~E.~S. and {Lyra}, W. and {Perets}, H.~B.},
	Date-Added = {2018-04-18 02:51:46 +0000},
	Date-Modified = {2018-04-18 02:51:58 +0000},
	Doi = {10.1111/j.1365-2966.2012.21486.x},
	Eprint = {1206.2309},
	Journal = {\mnras},
	Keywords = {accretion-discs, planets-disc interactions, protoplanetary discs, binaries:close, galaxies: active, galaxies:nuclei},
	Month = sep,
	Pages = {460-469},
	Title = {{Intermediate mass black holes in AGN discs - I. Production and growth}},
	Volume = 425,
	Year = 2012,
	Bdsk-Url-1 = {https://doi.org/10.1111/j.1365-2966.2012.21486.x}}

@article{horn,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750...34H},
	Archiveprefix = {arXiv},
	Author = {{Horn}, B. and {Lyra}, W. and {Mac Low}, M.-M. and {S{\'a}ndor}, Z.},
	Date-Added = {2018-04-18 02:49:18 +0000},
	Date-Modified = {2018-04-18 02:49:27 +0000},
	Doi = {10.1088/0004-637X/750/1/34},
	Eid = {34},
	Eprint = {1202.1868},
	Journal = {\apj},
	Keywords = {methods: numerical, planets and satellites: formation, planet-disk interactions, protoplanetary disks},
	Month = may,
	Pages = {34},
	Primaryclass = {astro-ph.EP},
	Title = {{Orbital Migration of Interacting Low-mass Planets in Evolutionary Radiative Turbulent Models}},
	Volume = 750,
	Year = 2012,
	Bdsk-Url-1 = {https://doi.org/10.1088/0004-637X/750/1/34}}

@article{lyra,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...715L..68L},
	Archiveprefix = {arXiv},
	Author = {{Lyra}, W. and {Paardekooper}, S.-J. and {Mac Low}, M.-M.},
	Date-Added = {2018-04-18 02:47:22 +0000},
	Date-Modified = {2018-04-18 02:47:51 +0000},
	Doi = {10.1088/2041-8205/715/2/L68},
	Eprint = {1003.0925},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, hydrodynamics, methods: numerical, planet-disk interactions, protoplanetary disks, radiation mechanisms: general},
	Month = jun,
	Pages = {L68-L73},
	Primaryclass = {astro-ph.EP},
	Title = {{Orbital Migration of Low-mass Planets in Evolutionary Radiative Models: Avoiding Catastrophic Infall}},
	Volume = 715,
	Year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1088/2041-8205/715/2/L68}}

@article{paardekooper2010,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401.1950P},
	Archiveprefix = {arXiv},
	Author = {{Paardekooper}, S.-J. and {Baruteau}, C. and {Crida}, A. and {Kley}, W.},
	Date-Added = {2018-04-18 02:45:35 +0000},
	Date-Modified = {2018-04-18 02:46:00 +0000},
	Doi = {10.1111/j.1365-2966.2009.15782.x},
	Eprint = {0909.4552},
	Journal = {\mnras},
	Keywords = {planets and satellites: formation, planetary systems: formation},
	Month = jan,
	Pages = {1950-1964},
	Primaryclass = {astro-ph.EP},
	Title = {{A torque formula for non-isothermal type I planetary migration - I. Unsaturated horseshoe drag}},
	Volume = 401,
	Year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1111/j.1365-2966.2009.15782.x}}

@article{paardekooper_mellema,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...459L..17P},
	Author = {{Paardekooper}, S.-J. and {Mellema}, G.},
	Date-Added = {2018-04-18 02:44:32 +0000},
	Date-Modified = {2018-04-18 02:44:56 +0000},
	Doi = {10.1051/0004-6361:20066304},
	Eprint = {astro-ph/0608658},
	Journal = {\aap},
	Keywords = {radiative transfer, hydrodynamics, methods: numerical, planets and satellites: formation},
	Month = nov,
	Pages = {L17-L20},
	Title = {{Halting type I planet migration in non-isothermal disks}},
	Volume = 459,
	Year = 2006,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361:20066304}}

@article{tanaka,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...565.1257T},
	Author = {{Tanaka}, H. and {Takeuchi}, T. and {Ward}, W.~R.},
	Date-Added = {2018-04-18 02:41:03 +0000},
	Date-Modified = {2018-04-18 02:41:38 +0000},
	Doi = {10.1086/324713},
	Journal = {\apj},
	Keywords = {Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks, Solar System: Formation, Waves},
	Month = feb,
	Pages = {1257-1274},
	Title = {{Three-Dimensional Interaction between a Planet and an Isothermal Gaseous Disk. I. Corotation and Lindblad Torques and Planet Migration}},
	Volume = 565,
	Year = 2002,
	Bdsk-Url-1 = {https://doi.org/10.1086/324713}}

@article{ward,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997Icar..126..261W},
	Author = {{Ward}, W.~R.},
	Date-Added = {2018-04-18 02:37:08 +0000},
	Date-Modified = {2018-04-18 02:37:20 +0000},
	Doi = {10.1006/icar.1996.5647},
	Journal = {\icarus},
	Month = apr,
	Pages = {261-281},
	Title = {{Protoplanet Migration by Nebula Tides}},
	Volume = 126,
	Year = 1997,
	Bdsk-Url-1 = {https://doi.org/10.1006/icar.1996.5647}}

@article{goldreich_tremaine,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...233..857G},
	Author = {{Goldreich}, P. and {Tremaine}, S.},
	Date-Added = {2018-04-18 02:34:57 +0000},
	Date-Modified = {2018-04-18 02:35:15 +0000},
	Doi = {10.1086/157448},
	Journal = {\apj},
	Keywords = {Density Wave Model, Galactic Structure, Rotating Disks, Astrodynamics, Hydrodynamics, Resonance, Stellar Motions, Wave Excitation},
	Month = nov,
	Pages = {857-871},
	Title = {{The excitation of density waves at the Lindblad and corotation resonances by an external potential}},
	Volume = 233,
	Year = 1979,
	Bdsk-Url-1 = {https://doi.org/10.1086/157448}}

@article{rodriguez,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016PhRvD..93h4029R},
	Archiveprefix = {arXiv},
	Author = {{Rodriguez}, C.~L. and {Chatterjee}, S. and {Rasio}, F.~A.},
	Date-Added = {2018-04-18 02:29:02 +0000},
	Date-Modified = {2018-04-18 02:29:15 +0000},
	Doi = {10.1103/PhysRevD.93.084029},
	Eid = {084029},
	Eprint = {1602.02444},
	Journal = {\prd},
	Month = apr,
	Number = 8,
	Pages = {084029},
	Primaryclass = {astro-ph.HE},
	Title = {{Binary black hole mergers from globular clusters: Masses, merger rates, and the impact of stellar evolution}},
	Volume = 93,
	Year = 2016,
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.93.084029}}

@article{Antonini_rasio,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831..187A},
	Archiveprefix = {arXiv},
	Author = {{Antonini}, F. and {Rasio}, F.~A.},
	Date-Added = {2018-04-18 02:25:46 +0000},
	Date-Modified = {2018-04-18 02:26:02 +0000},
	Doi = {10.3847/0004-637X/831/2/187},
	Eid = {187},
	Eprint = {1606.04889},
	Journal = {\apj},
	Keywords = {galaxies: nuclei, gravitational waves, stars: black holes},
	Month = nov,
	Pages = {187},
	Primaryclass = {astro-ph.HE},
	Title = {{Merging Black Hole Binaries in Galactic Nuclei: Implications for Advanced-LIGO Detections}},
	Volume = 831,
	Year = 2016,
	Bdsk-Url-1 = {https://doi.org/10.3847/0004-637X/831/2/187}}

@article{abbott,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...833L...1A},
	Archiveprefix = {arXiv},
	Author = {{Abbott}, B.~P. and {Abbott}, R. and {Abbott}, T.~D. and {Abernathy}, M.~R. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adams}, T. and {Addesso}, P. and {Adhikari}, R.~X. and et al.},
	Date-Added = {2018-03-25 16:30:02 +0000},
	Date-Modified = {2018-03-25 16:31:29 +0000},
	Doi = {10.3847/2041-8205/833/1/L1},
	Eid = {L1},
	Eprint = {1602.03842},
	Journal = {\apjl},
	Keywords = {black holes, gravitational waves, stars: massive},
	Month = dec,
	Pages = {L1},
	Primaryclass = {astro-ph.HE},
	Title = {{The Rate of Binary Black Hole Mergers Inferred from Advanced LIGO Observations Surrounding GW150914}},
	Volume = 833,
	Year = 2016,
	Bdsk-Url-1 = {https://dx.doi.org/10.3847/2041-8205/833/1/L1}}

@article{bellovary,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...819L..17B},
	Archiveprefix = {arXiv},
	Author = {{Bellovary}, J.~M. and {Mac Low}, M.-M. and {McKernan}, B. and {Ford}, K.~E.~S.},
	Date-Added = {2018-03-25 16:27:51 +0000},
	Date-Modified = {2018-03-25 16:31:19 +0000},
	Doi = {10.3847/2041-8205/819/2/L17},
	Eid = {L17},
	Eprint = {1511.00005},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, black hole physics, galaxies: nuclei},
	Month = mar,
	Pages = {L17},
	Title = {{Migration Traps in Disks around Supermassive Black Holes}},
	Volume = 819,
	Year = 2016,
	Bdsk-Url-1 = {https://dx.doi.org/10.3847/2041-8205/819/2/L17}}

@article{OLeary,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.395.2127O},
	Archiveprefix = {arXiv},
	Author = {{O'Leary}, R.~M. and {Kocsis}, B. and {Loeb}, A.},
	Date-Added = {2018-03-25 16:26:21 +0000},
	Date-Modified = {2018-03-25 16:31:14 +0000},
	Doi = {10.1111/j.1365-2966.2009.14653.x},
	Eprint = {0807.2638},
	Journal = {\mnras},
	Keywords = {black hole physics , gravitational waves , galaxies: kinematics and dynamics , galaxies: nuclei},
	Month = jun,
	Pages = {2127-2146},
	Title = {{Gravitational waves from scattering of stellar-mass black holes in galactic nuclei}},
	Volume = 395,
	Year = 2009,
	Bdsk-Url-1 = {https://dx.doi.org/10.1111/j.1365-2966.2009.14653.x}}

@article{Hopman:2006aa,
	Author = {Clovis Hopman and Tal Alexander},
	Date-Added = {2018-03-25 16:19:48 +0000},
	Date-Modified = {2018-03-25 16:19:48 +0000},
	Eprint = {astro-ph/0603324},
	Journal = {Astrophys.J.},
	Pages = {L133-L136},
	Title = {The effect of mass-segregation on gravitational wave sources near massive black holes},
	Url = {https://arxiv.org/abs/astro-ph/0603324},
	Volume = {645},
	Year = {2006},
	Bdsk-Url-1 = {https://arxiv.org/abs/astro-ph/0603324}}

@article{Sirko:2003aa,
	Author = {Edwin Sirko and Jeremy Goodman},
	Date-Added = {2018-03-25 16:09:24 +0000},
	Date-Modified = {2018-03-25 16:09:24 +0000},
	Eprint = {astro-ph/0209469},
	Journal = {Mon.Not.Roy.Astron.Soc.},
	Pages = {501},
	Title = {Spectral energy distributions of selfgravitating QSO discs},
	Url = {https://arxiv.org/abs/astro-ph/0209469},
	Volume = {341},
	Year = {2003},
	Bdsk-Url-1 = {https://arxiv.org/abs/astro-ph/0209469}}

